Tele-Aloha: A Low-budget and High-authenticity Telepresence System Using Sparse RGB Cameras

In this paper, we present a low-budget and high-authenticity bidirectional telepresence system, Tele-Aloha, targeting peer-to-peer communication scenarios. Compared to previous systems, Tele-Aloha utilizes only four sparse RGB cameras, one consumer-grade GPU, and one autostereoscopic screen to achieve high-resolution (2048x2048), real-time (30 fps), low-latency (less than 150ms) and robust distant communication. As the core of Tele-Aloha, we propose an efficient novel view synthesis algorithm for upper-body. Firstly, we design a cascaded disparity estimator for obtaining a robust geometry cue. Additionally a neural rasterizer via Gaussian Splatting is introduced to project latent features onto target view and to decode them into a reduced resolution. Further, given the high-quality captured data, we leverage weighted blending mechanism to refine the decoded image into the final resolution of 2K. Exploiting world-leading autostereoscopic display and low-latency iris tracking, users are able to experience a strong three-dimensional sense even without any wearable head-mounted display device. Altogether, our telepresence system demonstrates the sense of co-presence in real-life experiments, inspiring the next generation of communication.

==> mainbody.tex <==
\input{introduction}

\input{related-work}

\input{system-overview}

\input{rendering.tex}

\input{analysis}

\input{conclusion}

% Bibliography
\bibliographystyle{ACM-Reference-Format}
\bibliography{bibliography}

\begin{figure*}
    \centering
    \includegraphics[width=.85\linewidth]{asset/big_result1.jpg}
    \caption{Main results of Tele-Aloha system. The first column shows 2 of 4 input views. The first two rows show the results of static scenes. The other rows show the results of dynamic scenes. }
    \label{fig:mainresults}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.99\linewidth]{asset/things_inter-3row.pdf}
    \caption{Results of Tele-Aloha system on human-object interaction scenes. Our method can synthesis most of solid objects.}
    % \vspace{-2mm}
    \label{fig:objects}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.99\linewidth]{asset/failure-supp-long.pdf}
    \caption{Failure cases. Left one shows blurry eyeglasses. Right
        one shows that inaccuracy of background matting causes artifacts in novel views.}
    % \vspace{-2mm}
    \label{fig:failure_supp}
\end{figure*}









==> novel-view-synthesis.tex <==
\section{Novel view synthesis}
